Optimism for Boosting Concurrency

Modern concurrent programming benefits from a large variety of synchronization techniques. These include conventional pessimistic locking, as well as optimistic techniques based on conditional synchronization primitives or transactional memory. Yet, it is unclear which of these approaches better leverage the concurrency inherent to multi-cores. In this paper, we compare the level of concurrency one can obtain by converting a sequential program into a concurrent one using optimistic or pessimistic techniques. To establish fair comparison of such implementations, we introduce a new correctness criterion for concurrent programs, defined independently of the synchronization techniques they use. We treat a program's concurrency as its ability to accept a concurrent schedule, a metric inspired by the theories of both databases and transactional memory. We show that pessimistic locking can provide strictly higher concurrency than transactions for some applications whereas transactions can provide strictly higher concurrency than pessimistic locks for others. Finally, we show that combining the benefits of the two synchronization techniques can provide strictly more concurrency than any of them individually. We propose a list-based set algorithm that is optimal in the sense that it accepts all correct concurrent schedules. As we show via experimentation, the optimality in terms of concurrency is reflected by scalability gains.

==> app-elastic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Relaxed optimistic implementation: proof of correctness}
%\section{Relaxed optimistic implementation of the list-based set}
\label{app:lltm}
%
%
Let $\alpha$ be an execution of $I^{RM}$ and $<_\alpha$
denote the total-order on events in $\alpha$.
For simplicity, we assume that $\alpha$ starts with an artificial
sequential execution of an insert operation $\pi_0$ that inserts $\ms{tail}$ and sets $\ms{head}.\ms{next}=\ms{tail}$. 
%Let $\alpha|c$ denote the subsequence of $\alpha$ obtained by removing all synchronization primitives and all events and primitives of aborted and incomplete transactions.
Let $H$ be the history exported by $\alpha$, where 
all reads and writes are sequential. 
We construct $H$ by associating a linearization point $\ell_{op}$ with each
non-aborted read or write operation $op$ performed in $\alpha$  
as follows:
%
\begin{itemize}
\item  if $op$ is a read, then performed by process $p_k$,
  $\ell_{op}$ is the base-object $\lit{read}$ in line~\ref{line:linr};
\item  if $op$ is a write within an $\lit{insert}$ operation,
  $\ell_{op}$ is the base-object $\lit{cas}$ in line~\ref{line:linw};
\item  if $op$ is a write  within a $\lit{remove}$ operation,
  $\ell_{op}$ is the base-object  $\lit{cas}$ in line~\ref{line:inswrite}.
\end{itemize}
%
We say that a $\lit{read}$ of an element $X$ within an operation $\pi$
is \emph{valid} in $H$ 
(we also say that $X$ is \emph{valid}) if 
%there exists an $\lit{insert}$ operation that performs $\lit{write}(X.\ms{next}=Y)$ such that
there does not exist any $\lit{remove}$ operation $\pi_1$ that \emph{deallocates} $X$ (removes $X$ from the list)
such that $\ell_{\pi_1.\lit{write}(X)} <_{\alpha}
\ell_{\pi.\lit{read}(X)}$. 
%
\begin{lemma}
\label{lem:invar1}
Let $\pi$ be any operation performing $\lit{read}(X)$ followed by $\lit{read}(Y)$ in $H$. 
Then (1) there exists an $\lit{insert}$ operation that sets $X.\ms{next}=Y$ prior to $\pi.\lit{read}(X)$, and
(2) $\pi.\lit{read}(X)$ and $\pi.\lit{read}(Y)$ are \emph{valid} in $H$.
%(2) no other update performs a $\lit{write}$ to $X$ after the $\lit{write}$ to $X$ by $\pi'$ and before the $\lit{read}$ of $X$ by $\pi$.   
\end{lemma}
%%
\begin{proof} 
Let $\pi$ be any operation in $I^{RM}$ that performs $\lit{read}(X)$ followed by $\lit{read}(Y)$.
If $X$ and $Y$ are \emph{head} and \emph{tail} respectively, $\ms{head}.\ms{next}=\ms{tail}$ (by assumption). Since no $\lit{remove}$ operation
deallocates the \emph{head} or \emph{tail}, the $\lit{read}$ of $X$ and $Y$ are \emph{valid} in $H$.

Now, let $X$ be the \emph{head} element and suppose that $\pi$ performs $\lit{read}(X)$ followed by $\lit{read}(Y)$; $Y\neq \ms{tail}$ in $H$.
Clearly, if $\pi$ performs a $\lit{read}(Y)$, there exists an
operation $\pi'=\lit{insert}$ that has previously set $\emph{head}.\ms{next}=Y$.
More specifically, $\pi.\lit{read}(X)$ performs the action in line~\ref{line:linr} after the
write to shared memory by $\pi'$ in line~\ref{line:inscommit}. 
%But $\pi'$ must have performed the action in line~\ref{line:linw} of $R$ prior to the write to shared memory in line~\ref{line:commit-update}.
By the assignment of linearization points to tx-operations, $\ell_{\pi'} <_{\alpha} \ell_{\pi.\lit{read}(X)}$.
Thus, there exists an $\lit{insert}$ operation that sets $X.\ms{next}=Y$ prior to $\pi.\lit{read}(X)$ in $H$.

For the second claim, we need to prove that the $\lit{read}(Y)$ by $\pi$ is \emph{valid} in $H$.
Suppose by contradiction that $Y$ has been deallocated by some $\pi''=\lit{remove}$ operation prior to $\lit{read}(Y)$ by $\pi$.
By the rules for linearization of read and write operations, the action in line~\ref{line:commit-update} precedes the action in line~\ref{line:linr}.
However, $\pi$ proceeds to perform the check in line~\ref{line:flagcheck} and returns $\bot$ since the flag corresponding to the element $Y$ is previously set by $\pi''$. Thus, $H$ does not contain $\pi.\lit{read}(Y)$---contradiction.
%An identical argument applied to element $Y$ also proves that $\lit{read}(Y)$ is \emph{valid} in $H$.

Inductively, by the above arguments, every non-\emph{head} $\lit{read}$ by $\pi$ 
is performed on an element previously created by an $\lit{insert}$ operation
and is valid in $H$.
\end{proof} 
%
\begin{lemma}
\label{lem:rls}
$H$ is locally serializable with respect to $\LL$.
\end{lemma}
%
\begin{proof}
%
By Lemma~\ref{lem:invar1}, every element $X$ read 
within an operation $\pi$ 
is previously created by an $\lit{insert}$ operation and is valid in $H$.
Moreover, if the read operation on $X$ returns $v'$, then 
$X.\textit{next}$ stores a pointer to another valid element that
stores an integer value $v''>v'$.
Note that the series of reads performed by $\pi$ terminates as soon as 
an element storing value $v$ or higher is found. Thus, $\pi$ performs at most
$O(|v-v_0|)$ reads, where $v_0$ is the value of the second element read by $\pi$.  
%By construction, any update operation in $I^{RM}$ performs at most two writes.
Now we construct $S^{\pi}$ as a sequence of $\lit{insert}$ operations,
that insert values read by $\pi$, one by one, followed by $\pi$. 
By construction, $S^{\pi}\in\Sigma_{\ms{LL}}$.
%Similarly, we can construct sequential histories for $\lit{insert}$ and $\lit{remove}$ operations that are consistent with their local histories.
\end{proof}
%
%\begin{proof}
%
%Since \emph{linearizability} is a \emph{safety}
%property~\cite{Lyn96}, 
It is sufficient for us to prove that every finite high-level history $H$
of $I^{RM}$ is linearizable.
%We now prove that every finite high-level history $\tilde H$ of $I^H$ is linearizable.
%
First, we obtain a completion $\tilde H$ of $H$ as follows.
%the high-level history corresponding to $\alpha$ 
%by performing the following actions on operations that are incomplete in $H$.
The invocation of an incomplete \lit{contains} operation is discarded.
The invocation of an incomplete $\pi=\lit{insert} \vee \lit{remove}$
operation that has not returned successfully from the $\lit{write}$
operation is discarded; otherwise, it is completed with response $\true$.
%

We obtain a sequential high-level history $\tilde S$ equivalent to $\tilde H$ by associating a linearization point $\ell_{\pi}$ 
with each operation $\pi$ as follows.
For each $\pi=\lit{insert}\vee\lit{remove}$ that returns $\true$ in $\tilde H$, $\ell_{\pi}$ is associated with 
%the last step of the \emph{tryCommit} (line~\ref{line:end-commit} of Algorithm~\ref{alg:elastic}) invoked in 
the first $\lit{write}$ performed by $\pi$ in $H$; otherwise
$\ell_{\pi}$ is associated with the last $\lit{read}$ performed by $\pi$ in $H$. For $\pi=\lit{contains}$ that returns $\true$, $\ell_{\pi}$
is associated with the last $\lit{read}$ performed in $I^{RM}$; otherwise $\ell_{\pi}$ is associated with the $\lit{read}$ of \emph{head}.
%
Since linearization points are chosen within the intervals of 
operations of $I^{RM}$, for any two operations
$\pi_i$ and $\pi_j$ in ${\tilde H}$, if $\pi_i \rightarrow_{\tilde H}
\pi_j$, then $\pi_i \rightarrow_{\tilde S} \pi_j$.
%
\begin{lemma}
\label{lem:rlegal}
$\tilde S$ is consistent with the sequential specification of type \textit{set}.
\end{lemma}
\begin{proof}
%
Let ${\tilde S}^k$ be the prefix of $\tilde S$ consisting of
the first $k$ complete operations. 
%(last event of ${\tilde S}^k$ is a response event).
%The state of the \emph{set} object at ${\tilde S}^0$ is $\emptyset$.
We associate each ${\tilde S}^k$ with a set $q^k$ of objects that were
successfully inserted and not subsequently successfully removed in ${\tilde S}^k$.
We show by induction on $k$ that the sequence of state transitions in
${\tilde S}^k$ is consistent with operations' responses in ${\tilde
  S}^k$ with respect to the \textit{set} type. 

%To prove that ${\tilde S}$ indeed consistent with \emph{set}, we
%proceed by induction on $k$. 
The base case $k=1$ is trivial: the \textit{tail} element containing
$+\infty$ is successfully inserted.
Suppose that ${\tilde S}^k$ is consistent with the \emph{set} type and
let $\pi_1$ with argument $v\in \mathbb{Z}$ and response $r_{\pi_{1}}$
be the last operation of ${\tilde S}^{k+1}$.  
We want to show that $(q^k,\pi_1,q^{k+1},r_{\pi_{1}})$ is consistent with the \textit{set} type. 
%We now prove that, upon the invocation of an operation $\pi_1$ with argument $v\in \mathbb{Z}$ applied at ${\tilde S}^k$ in state $q \in 2^{\mathbb{Z}}$,
%$(q,\pi_1,q',r_{\pi_{1}})$ is contained in the sequential
%specification of the \emph{set} type, where $q'$ is content of the
%\emph{set} object after ${\tilde S}^{k+1}$ defined in a natural way. We then say that ${\tilde S}^{k+1}$ satisfies $(q,\pi_1(v),q',r_{\pi_1})$.
%
%Let ${\tilde S}^k$ be the complete prefix of $\tilde S$ of length $k$.
%We proceed by induction on $k$.
%Let $\pi_1$ with argument $v\in \mathbb{Z}$ be the operation of the \emph{set} type applied at ${\tilde S}^k$ in state $q \in \mathbb{Z}$.
%
\begin{enumerate}
\item[(1)]
If $\pi_1=\lit{insert}(v)$ returns $\true$ in ${\tilde S}^{k+1}$, there does not exist any other $\pi_2=\lit{insert}(v)$ that returns $\true$ in ${\tilde S}^{k+1}$ such that there does not exist any $\lit{remove}(v)$ that returns $\true$; $\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
Suppose by contradiction that such a $\pi_1$ and $\pi_2$ exist.
Every successful $\lit{insert}(v)$ operation performs its penultimate $\lit{read}$ on an element $X$ that stores a value $v'<v$ and the last read is performed on an element that stores a value $v''>v$. Clearly, $\pi_1$ also performs a $\lit{write}$ on $X$.
By construction of $\tilde S$, $\pi_1$ is linearized at the release of the \emph{cas} lock on element $X$.
Observe that $\pi_2$ must also perform a $\lit{write}$ to the element $X$ (otherwise one of $\pi_1$ or $\pi_2$ would return $\false$).
By assumption, the write to $X$ in shared-memory by $\pi_2$
(line~\ref{line:inscommit}) precedes the corresponding write to $X$ in
shared-memory by $\pi_2$. If $\ell_{\pi_2} <_{\alpha}
\ell_{\pi_{1}.\lit{read}(X)}$, then $\pi_1$ cannot return $\true$---a contradiction.
Otherwise, if $\ell_{\pi_{1}.\lit{read}(X)}  <_{\alpha} \ell_{\pi_2}$,
then $\pi_1$ reaches line~\ref{line:linw} and return
$\bot$. This is because either $\pi_1$ attempts to acquire the
\emph{cas} lock on $X$ while it is still held by $\pi_2$ or the value
of $X$ contained in the \emph{rbuf} of the process executing $\pi_1$
has changed---a contradiction. 

If $\pi_1=\lit{insert}(v)$ returns $\false$ in ${\tilde S}^{k+1}$, there exists a $\pi_2=\lit{insert}(v)$ that returns $\true$ in ${\tilde S}^{k+1}$ such that there does not exist any $\pi_3=\lit{remove}(v)$ that returns $\true$; $\pi_2 \rightarrow_{{\tilde S}^{k+1}} \pi_3 \rightarrow_{{\tilde S}^{k+1}} \pi_1$. 
Suppose that such a $\pi_2$ does not exist. Thus, $\pi_1$ must perform
its last $\lit{read}$ on an element that stores value $v''>v$, perform
the action in Line~\ref{line:inscommit} and return $\true$---a contradiction.

It is easy to verify that the conjunction of the above two claims prove that $\forall q\in Q$; $\forall v\in \mathbb{Z}$, ${\tilde S}^{k+1}$ satisfies $(q,\lit{insert}(v),q \cup \{v\},(v \not\in q))$.
\item[(2)]
If $\pi_1=\lit{remove}(v)$, similar arguments as applied to $\lit{insert}(v)$ prove that $\forall q\in Q$; $\forall v\in \mathbb{Z}$, ${\tilde S}^{k+1}$ satisfies $(q,\lit{remove}(v),q \setminus \{v\},(v \in q))$.

\item[(3)]
If $\pi_1=\lit{contains}(v)$ returns $\true$ in ${\tilde S}^{k+1}$, there exists $\pi_2=\lit{insert}(v)$ that returns \emph{true} in ${\tilde S}^{k+1}$ such that there does not exist any $\lit{remove}(v)$ that returns \emph{true} in ${\tilde S}^{k+1}$ such that $\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
The proof of this claim immediately follows from Lemma~\ref{lem:invar1}.
%Observe that the check in line~\ref{line:ccheck} of $I^{RM}$ returns $\true$ only if there exists an element that stores value $v$.
%Indeed, there exists an $\lit{insert}(v)$ that writes the value $v$ to some element and updated in shared-memory (line~\ref{line:commit-update} of $R$). Note that $\ell_{\pi_2}$ is associated with the action performed in line~\ref{line:commit-update} of $R$ by $\pi_2$ and
%$\ell_{\pi_1}$ is associated with the action in line~\ref{line:linr} of $R$ performed by the last $\lit{read}$ by $\pi_1$.
%Thus, $\pi_2 \rightarrow_{\tilde S} \pi_1$.
%Now, suppose by contradiction that there exists a $\lit{remove}(v)$ that returns \emph{true} in $\tilde S$ such that $\pi_2 \rightarrow_{\tilde S} \lit{remove}(v) \rightarrow_{\tilde S} \pi_1$. 
%Then, $\ell_{\pi_2} <_{\alpha} \ell_{\lit{remove}(v)}$ $<_{\alpha}$ $\ell_{\pi_1}$. 
%By the assignment of linearization points, $\lit{contains}(v)$ performs the read in line~\ref{line:linr} in $R$ after the last write to shared memory by $\pi_1$. But then, due to the check in line~\ref{line:flagcheck} of $R$, $\lit{contains}(v)$ cannot return $\true$---contradiction.

Now, if $\pi_1=\lit{contains}(v)$ returns $\false$ in ${\tilde S}^{k+1}$, 
there does not exist an $\pi_2=\lit{insert}(v)$ that returns \emph{true} such that 
%$\lit{insert}(v) \rightarrow_{S} \lit{contains}(v)$ or 
there does not exist any $\lit{remove}(v)$ that returns \emph{true}; 
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \lit{contains}(v)$.
Suppose by contradiction that such a $\pi_1$ and $\pi_2$ exist. 
%We argue that the only possibility then is the $\lit{contains}$ operation traverses the entire list without finding the element that stores value $v$.
Thus, the action in line~\ref{line:inscommit} by the $\lit{insert}(v)$ operation that updates some element, 
say $X$ precedes the action in line~\ref{line:linr} by $\lit{contains}(v)$ that is associated with its 
first $\lit{read}$ (the \emph{head}).
We claim that $\lit{contains}(v)$ must read the element $X'$ newly created by
$\lit{insert}(v)$ and return $\true$---a contradiction to the initial assumption that it returns $\false$.
The only case when this can happen is if there exists a $\lit{remove}$
operation that forces $X'$ to be unreachable from \emph{head} i.e. concurrent to the $\lit{write}$
to $X$ by $\lit{insert}$, there exists a $\lit{remove}$ that sets $X''.\textit{next}$ to $X.\textit{next}$
after the action in line~\ref{line:inswrite} by $\lit{insert}$.
But this is not possible since the \emph{cas} on $X$ performed by the $\lit{remove}$
would return $\false$.
%
\end{enumerate}
%
Thus, inductively, the sequence of state transitions in ${\tilde S}$
satisfies the sequential specification of the \textit{set} type. 
\end{proof}
%
Lemmas~\ref{lem:rls} and~\ref{lem:rlegal} imply:
%
\begin{theorem}
\label{th:lr}
$I^{RM}$ is \LS-linearizable with respect to $(\LL,\ms{set})$.
\end{theorem}
%
%\begin{corollary}
%\label{cr:rel}
%$I^{RM}\in \mathcal{RM}$.
%\end{corollary}
%%
%\begin{proof}
%%
%Consider the schedule $\sigma_0$ depicted in Figure~\ref{fig:ex1}.
%It cannot be exported by any implementation based on a safe-strict serializable TM.
%However, there exists an execution of $I^{RM}$ that exports $\sigma_0$ (by Lemma~\ref{lem:lrelaxed}).
%
%The proof now follows from Theorem~\ref{th:lr}.
%\end{proof}
%
% \begin{theorem}
% \label{th:nbll}
% %
% $I^{RM}$ is a non-blocking implementation of $(\LL,\ms{set})$.
% \end{theorem}
% %
% \begin{proof}
% %
% Suppose that any operation $\pi$ fails to return a matching response i.e.
% returns $\bot$ as it performs a read of some object $X$ from line~\ref{line:flagcheck}.
% Thus, there exists an $\lit{insert}$ that has performed the action in line~\ref{line:inscommit} during
% a $\lit{write}$ to $X$
% or there exists a $\lit{remove}$
% that has performed one of the actions, line~\ref{line:elastic:gc} or line~\ref{line:commit-update}
% prior to the action in line~\ref{line:flagcheck} by $\pi$.
% In all cases, the concurrent $lit{insert}$ or $\lit{remove}$ must terminate and return a matching response.
% 
% Suppose that an $\lit{insert}$ operation $\pi$ returns $\bot$ in line~\ref{line:inswrite} while
% performing a $\lit{write}$ on some object $X$.
% Thus, there exists a concurrent operation $\pi'$ that 
% performs a $\lit{write}$ to $X$ after the $\lit{read}$ of $X$ by $\pi$.
% If $\pi'$ is an $\lit{insert}$, then $\pi'$ must terminate and return a matching response.
% Otherwise if $\pi'$ is a $\lit{remove}$ operation, consider two cases:
% (1) $\pi'$ has performed the action in line~\ref{line:linw} to return successfully from the \emph{cas}
% on $X$ or (2) $\pi'$ has performed the action in line~\ref{line:linw2} to
% return successfully from the \emph{cas}
% on $X$. In case $(1)$, 
% 
% Suppose that a $\lit{remove}$ operation $\pi$ returns $\bot$ in line~\ref{line:linw} while
% performing a $\lit{write}$ on some object $X$.
% 
% Suppose that a $\lit{remove}$ operation $\pi$ returns $\bot$ in line~\ref{line:linw2} while
% performing a $\lit{write}$ on some object $X$.
% \end{proof}
% %


==> sequential.tex <==
\begin{algorithm*}[ht]
\caption{Sequential implementation {\LL} (\textit{sorted linked list}) of \emph{set} type}
\label{alg:lists}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\size
	
	\Part{Shared variables}{
%		\State Objects $X_i$; $i\in \mathbb{N}$
%		~~~~~\State $X_i.next$
%		~~~~~\State $X_i.val$
		\State Initially $\ms{head}$, $\ms{tail}$,
		\State ~~~$\ms{head}.val=-\infty$, $\ms{tail}.val=+\infty$
		\State ~~~$\ms{head}.next=\ms{tail}$
	}\EndPart
	
	\Statex
	
	\Part{$\lit{insert}(v$)}{
		%\State $\tup{\ms{prev}, \ms{curr}} \gets \lit{locate}(v)$
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
		\While{$\ms{new.val} < v $} 
			\State $\ms{prev} \gets \ms{curr}$
			\State $\ms{old}\gets \ms{new}$
			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{new} \gets \lit{read}(\ms{curr})$
		\EndWhile
		\If{$\ms{new.val} \neq v$}
			\State $X \gets \lit{new-node}(v,\ms{curr})$ \Comment{local action}
			%\State $X.\ms{next} \gets \ms{curr}$
			\State $\lit{write}(\ms{prev},[\ms{old.val},X])$ 
			%\State $\ms{result} \gets \lit{true}$
%		\Else
%			\State $\ms{result} \gets \lit{false}$
		\EndIf
		\Return $(\ms{new.val}\neq v)$ \EndReturn
   	}\EndPart
	
	\newpage
	%\Statex
	\Part{$\lit{remove}(v$)}{
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
		\While{$\ms{new.val} < v $} 
			\State $\ms{prev} \gets \ms{curr}$
			\State $\ms{old} \gets \ms{new}$
			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{new} \gets \lit{read}(\ms{curr})$
		\EndWhile
		%\State $\tup{\ms{prev}, \ms{curr}} \gets \lit{locate}(v)$
 	 	\If{$\ms{new.val}  = v$}
			%\State $\ms{curr.marked} \gets \lit{true}$ 
			%\State\Comment{Mark node for removal}
			\State $\lit{write}(\ms{prev} ,[\ms{old.val},\ms{new.next}])$
			%\State $\lit{write}(\ms{curr}, [\bot,\bot])$ \Comment{write $\bot$ to \emph{val} and \emph{next} fields}
			%\State $\ms{result} \gets \lit{true}$
%		\Else
%			\State $\ms{result} \gets \lit{false}$
		\EndIf
		\Return $(\ms{new.val}=v)$ \EndReturn
   	}\EndPart
	
	\Statex
	
	\Part{$\lit{contains}(v$)}{
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
		\While{$\ms{new.val} < v $} 
			\State $\ms{prev} \gets \ms{curr}$
			\State $\ms{old}\gets \ms{new}$
			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{new} \gets \lit{read}(\ms{curr})$
		\EndWhile
		%\State $\tup{\ms{prev}, \ms{curr}} \gets \lit{locate}(v)$
		%\If{$\ms{t.val} = v$}
%			\State $\ms{result} \gets \lit{true}$
%		\Else
%			\State $\ms{result} \gets \lit{false}$
 	   	\Return $(\ms{new.val}=v)$ \EndReturn	
 	   	%\EndIf
   	 }\EndPart

		
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}


==> tline.tex <==
\begin{tikzpicture}
%%\node (b1) at (2,0) [fill,circle,inner sep=2.2pt] {};
%%\node (b2) at (-1,-1) [fill,circle,inner sep=2.2pt] {};
%%\node (b3) at (-1.8,-2) [fill,circle,inner sep=2.2pt] {};
%
\node (r1) at (2,0) [fill,circle,inner sep=1.5pt] {};
\node (r2) at (7,0) [fill,circle,inner sep=1.5pt] {};
\node (w1) at (4.5,-1) [fill,circle,inner sep=1.5pt] {};

\draw (r1) node [below] {\tiny {$R(X_1)$}}
   %(c2) node [below] {\tiny {$W_2(X_4)$}}
   (r2) node [below] {\tiny {$R(X_{k})$}};
   
\draw (w1) node [below] {\tiny {$W(X_i)$}};
 
\begin{scope}   
\draw [|-|,thick] (1.5,0) node[left] {$Contains(k)$} to (7.5,0);
\end{scope}
\begin{scope}
\draw [|-|,thick] (4,-1) node[left] {$Insert(j)$} to (5,-1) ; 
\end{scope}  
%
\end{tikzpicture}

